Factor Graph Optimization of Error-Correcting Codes for Belief Propagation Decoding

The design of optimal linear block codes capable of being efficiently decoded is of major concern, especially for short block lengths. As near capacity-approaching codes, Low-Density Parity-Check (LDPC) codes possess several advantages over other families of codes, the most notable being its efficient decoding via Belief Propagation. While many LDPC code design methods exist, the development of efficient sparse codes that meet the constraints of modern short code lengths and accommodate new channel models remains a challenge. In this work, we propose for the first time a gradient-based data-driven approach for the design of sparse codes. We develop locally optimal codes with respect to Belief Propagation decoding via the learning of the Factor graph under channel noise simulations. This is performed via a novel complete graph tensor representation of the Belief Propagation algorithm, optimized over finite fields via backpropagation and coupled with an efficient line-search method. The proposed approach is shown to outperform the decoding performance of existing popular codes by orders of magnitude and demonstrates the power of data-driven approaches for code design.

==> Tables/table_large_codes.tex <==
\begin{table}[h]
    \centering
    \caption{
    A comparison of the negative natural logarithm of Bit Error Rate (BER) for several normalized SNR values of our method with classical codes. Higher is better. BP results are provided for 5 iterations in the first row and 15 in the second row. The best results are in bold.}
    \label{tab:main_ber}
    % \setlength\tabcolsep{1.5pt}
%    \smallskip
% \vspace{-2mm}
    \resizebox{0.99985\textwidth}{!}{%
    \begin{tabular}{@{}lc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}c@{}}
    \toprule
        Channel & \multicolumn{10}{c}{AWGN} & \multicolumn{10}{c}{Fading} & \multicolumn{10}{c}{Bursting}\\
  %       \cmidrule(lr){2-4}
  %       \cmidrule(lr){5-13}
		% \cmidrule(lr){14-16}
        Method & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} &  \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} \\
  %       \cmidrule(lr){2-4}
  %       \cmidrule(lr){5-7}
  %       \cmidrule(lr){8-10}
  %       \cmidrule(lr){11-13}
		% \cmidrule(lr){14-16}
         $E_{b}/N_{0}$ & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7  \\ 
         \midrule                                                                                                                                                                                                                                                                                                                                                                                                                                      
		%%%%%%%%%%%%%%%%%%%
 
TANNER(155,64)  \comment{AWGN} \comment{BP} & \makecell{5 .16\\5.83} & \makecell{7.62\\8.54} & \makecell{10.92\\12.14} & \makecell{14.65\\ \bf16.50} & \makecell{17.63\\ \bf18.28} \comment{Our} & \makecell{\bf5.31\\ \bf6.32} & \makecell{\bf7.78\\ \bf9.20} & \makecell{\bf11.03\\ \bf12.89} & \makecell{\bf14.83\\16.36} & \makecell{\bf18.04\\18.20} \comment{Fading_1.0} \comment{BP} & \makecell{6.26\\7.29} & \makecell{8.14\\9.56} & \makecell{10.37\\12.07} & \makecell{12.48\\ \bf14.84} & \makecell{14.73\\ \bf16.91} \comment{Our} & \makecell{\bf6.34\\ \bf7.57} & \makecell{\bf8.25\\ \bf9.79} & \makecell{\bf10.42\\ \bf12.29} & \makecell{\bf12.62\\14.71} & \makecell{\bf14.94\\16.77} \comment{Bursting} \comment{BP} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} \comment{Our} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} \\ \midrule

WIMAX(192,96)   \comment{AWGN} \comment{BP} & \makecell{5.72\\ \bf7.09} & \makecell{8.72\\ \bf10.90} & \makecell{\bf12.68\\15.55} & \makecell{17.04\\ \bf18.19} & \makecell{18.60\\18.72} \comment{Our} & \makecell{\bf5.73\\7.07} & \makecell{\bf8.73\\10.86} & \makecell{12.54\\ \bf15.66} & \makecell{\bf17.09\\17.97} & \makecell{\bf18.79\\ \bf18.74} \comment{Fading_1.0} \comment{BP} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} \comment{Our} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} & \makecell{\bf-6.91\\ \bf-6.91} \comment{Bursting} \comment{BP} & \makecell{4.70\\5.73} & \makecell{\bf7.15\\8.97} & \makecell{\bf10.53\\ \bf12.99} & \makecell{\bf14.45\\17.00} & \makecell{\bf18.10\\18.47} \comment{Our} & \makecell{\bf4.70\\ \bf5.74} & \makecell{7.15\\ \bf8.99} & \makecell{10.45\\12.84} & \makecell{14.31\\ \bf17.13} & \makecell{18.07\\ \bf18.62} \\ \midrule

WRAN(480,400)   \comment{AWGN} \comment{BP} & \makecell{4.18\\4.38} & \makecell{6.95\\7.79} & \makecell{\bf11.45\\ \bf12.86} & \makecell{16.74\\ \bf18.23} & \makecell{20.32\\ \bf20.52} \comment{Our} & \makecell{\bf4.19\\ \bf4.39} & \makecell{\bf6.96\\ \bf7.79} & \makecell{11.43\\12.82} & \makecell{\bf16.77\\18.16} & \makecell{\bf20.61\\20.36} \comment{Fading_1.0} \comment{BP} \comment{Our} \comment{Bursting} \comment{BP} & \makecell{\bf3.38\\3.41} & \makecell{\bf4.85\\ \bf5.24} & \makecell{\bf7.84\\ \bf8.90} & \makecell{11.93\\13.39} & \makecell{\bf16.58\\17.95} \comment{Our} & \makecell{3.38\\ \bf3.41} & \makecell{4.85\\5.24} & \makecell{7.82\\8.89} & \makecell{\bf12.01\\ \bf13.59} & \makecell{16.50\\ \bf18.13} \\



\bottomrule
	\end{tabular}
	}
\end{table} 


==> Tables/table_pge.tex <==
\begin{table}[h]
    \centering
    \caption{
    A comparison of the negative natural logarithm of Bit Error Rate (BER) for several normalized SNR values of our method with classical PGE sparse codes. Here PGE$X$ means the degree of each node is of $X\%$. Higher is better. BP results are provided for 5 iterations in the first row and 15 in the second row. The best results are in bold.}
    \label{tab:pge}
    % \setlength\tabcolsep{1.5pt}
%    \smallskip
% \vspace{-2mm}
    \resizebox{0.99985\textwidth}{!}{%
    \begin{tabular}{@{}lc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}c@{}}
    \toprule
        Channel & \multicolumn{10}{c}{AWGN} & \multicolumn{10}{c}{Fading} & \multicolumn{10}{c}{Bursting}\\
  %       \cmidrule(lr){2-4}
  %       \cmidrule(lr){5-13}
		% \cmidrule(lr){14-16}
        Method & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} &  \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} \\
  %       \cmidrule(lr){2-4}
  %       \cmidrule(lr){5-7}
  %       \cmidrule(lr){8-10}
  %       \cmidrule(lr){11-13}
		% \cmidrule(lr){14-16}
         $E_{b}/N_{0}$ & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7  \\ 
         \midrule                                                                                                                                                                                                                                                                                                                                                                                                                                      
		%%%%%%%%%%%%%%%%%%%

PGE2(64,32)     \comment{AWGN} \comment{BP} & \makecell{3.78\\3.78} & \makecell{4.38\\4.38} & \makecell{5.12\\5.13} & \makecell{6.04\\6.04} & \makecell{7.17\\7.16} \comment{Our} & \makecell{\bf3.84\\ \bf3.84} & \makecell{\bf4.45\\ \bf4.44} & \makecell{\bf5.19\\ \bf5.19} & \makecell{\bf6.10\\ \bf6.10} & \makecell{\bf7.22\\ \bf7.23} \comment{Fading_1.0} \comment{BP} & \makecell{3.74\\3.74} & \makecell{4.08\\4.08} & \makecell{4.44\\4.44} & \makecell{4.81\\4.81} & \makecell{5.20\\5.20} \comment{Our} & \makecell{\bf3.75\\ \bf3.75} & \makecell{\bf4.10\\ \bf4.10} & \makecell{\bf4.46\\ \bf4.47} & \makecell{\bf4.85\\ \bf4.85} & \makecell{\bf5.24\\ \bf5.24} \comment{Bursting} \comment{BP} & \makecell{\bf3.54\\ \bf3.54} & \makecell{4.07\\4.06} & \makecell{4.69\\4.69} & \makecell{5.43\\5.43} & \makecell{6.29\\6.29} \comment{Our} & \makecell{\bf3.54\\ \bf3.54} & \makecell{\bf4.07\\ \bf4.06} & \makecell{\bf4.70\\ \bf4.69} & \makecell{\bf5.43\\ \bf5.44} & \makecell{\bf6.30\\ \bf6.30} \\ \midrule

PGE5(64,32)     \comment{AWGN} \comment{BP} & \makecell{4.41\\4.78} & \makecell{6.02\\6.63} & \makecell{8.20\\9.06} & \makecell{10.95\\ \bf12.30} & \makecell{14.40\\ \bf15.75} \comment{Our} & \makecell{\bf4.82\\ \bf5.26} & \makecell{\bf6.53\\ \bf7.13} & \makecell{\bf8.73\\ \bf9.48} & \makecell{\bf11.56\\12.20} & \makecell{\bf14.41\\14.90} \comment{Fading_1.0} \comment{BP} & \makecell{4.56\\4.98} & \makecell{5.63\\6.19} & \makecell{6.86\\7.52} & \makecell{8.31\\9.02} & \makecell{9.78\\10.76} \comment{Our} & \makecell{\bf5.09\\ \bf5.67} & \makecell{\bf6.22\\ \bf6.96} & \makecell{\bf7.48\\ \bf8.34} & \makecell{\bf8.82\\ \bf9.85} & \makecell{\bf10.16\\ \bf11.24} \comment{Bursting} \comment{BP} & \makecell{3.84\\4.13} & \makecell{5.18\\5.68} & \makecell{6.97\\7.75} & \makecell{9.34\\ \bf10.19} & \makecell{\bf12.25\\ \bf13.40} \comment{Our} & \makecell{\bf4.19\\ \bf4.55} & \makecell{\bf5.59\\ \bf6.12} & \makecell{\bf7.41\\ \bf8.06} & \makecell{\bf9.51\\10.13} & \makecell{11.84\\12.27} \\ \midrule

  PGE10(64,32)    \comment{AWGN} \comment{BP} & \makecell{3.08\\3.20} & \makecell{3.98\\4.27} & \makecell{5.17\\5.77} & 
  \makecell{6.70\\7.67} & \makecell{8.49\\9.72} \comment{Our} & \makecell{\bf4.21\\ \bf4.62} & \makecell{\bf5.56\\ \bf6.25} & \makecell{\bf7.22\\ \bf8.28} & \makecell{\bf9.13\\ \bf10.59} & \makecell{\bf11.11\\ \bf12.84} \comment{Fading_1.0} \comment{BP} & \makecell{2.96\\3.08} & \makecell{3.52\\3.71} & \makecell{4.18\\4.47} & \makecell{4.95\\5.30} & \makecell{5.81\\6.24} \comment{Our} & \makecell{\bf4.16\\ \bf4.60} & \makecell{\bf5.02\\ \bf5.60} & \makecell{\bf6.00\\ \bf6.72} & \makecell{\bf7.11\\ \bf7.90} & \makecell{\bf8.33\\ \bf9.24} \comment{Bursting} \comment{BP} & \makecell{2.75\\2.82} & \makecell{3.48\\3.67} & \makecell{4.47\\4.90} & \makecell{5.75\\6.46} & \makecell{7.28\\8.26} \comment{Our} & \makecell{\bf3.30\\ \bf3.57} & \makecell{\bf4.26\\ \bf4.73} & \makecell{\bf5.50\\ \bf6.22} & \makecell{\bf7.01\\ \bf8.01} & \makecell{\bf8.80\\ \bf10.06} \\

\bottomrule
	\end{tabular}
	}
\end{table} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
%     \centering
%     \caption{
%     A comparison of the negative natural logarithm of Bit Error Rate (BER) for five normalized SNR values of our method with classical codes. Higher is better. BP results are provided for 5 iterations in the first row and 15 in the second row. The best results are in bold.}
%     \label{tab:main_ber}
%     % \setlength\tabcolsep{1.5pt}
% %    \smallskip
% % \vspace{-2mm}
%     \resizebox{0.99985\textwidth}{!}{%
%     \begin{tabular}{@{}lc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}cc@{~}c@{~}c@{~}c@{~}c@{}}
%     \toprule
%         Channel & \multicolumn{10}{c}{AWGN} & \multicolumn{10}{c}{Fading} & \multicolumn{10}{c}{Bursting}\\
%   %       \cmidrule(lr){2-4}
%   %       \cmidrule(lr){5-13}
% 		% \cmidrule(lr){14-16}
%         Method & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} & \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} &  \multicolumn{5}{c}{BP} & \multicolumn{5}{c}{Our} \\
%   %       \cmidrule(lr){2-4}
%   %       \cmidrule(lr){5-7}
%   %       \cmidrule(lr){8-10}
%   %       \cmidrule(lr){11-13}
% 		% \cmidrule(lr){14-16}
%          $E_{b}/N_{0}$ & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7 & 3 & 4 & 5 & 6 & 7  \\ 
%          \midrule                                                                                                                                                                                                                                                                                                                                                                                                                                      
% 		%%%%%%%%%%%%%%%%%%%%                                                                                                         
%   BCH(63,45)      \comment{AWGN} \comment{BP} & \makecell{3.35\\3.40} & \makecell{4.06\\4.21} & \makecell{4.91\\5.24} & \makecell{6.04\\6.59} & \makecell{7.47\\8.35} \comment{Our} & \makecell{\bf3.48\\ \bf3.57} & \makecell{\bf4.30\\ \bf4.50} & \makecell{\bf5.28\\ \bf5.68} & \makecell{\bf6.54\\ \bf7.14} & \makecell{\bf8.08\\ \bf9.04} \comment{Fading} \comment{BP} & \makecell{2.77\\2.79} & \makecell{3.09\\3.13} & \makecell{3.46\\3.55} & \makecell{3.90\\4.04} & \makecell{4.37\\4.61} \comment{Our} & \makecell{\bf2.80\\ \bf2.83} & \makecell{\bf3.14\\ \bf3.20} & \makecell{\bf3.54\\ \bf3.65} & \makecell{\bf4.00\\ \bf4.18} & \makecell{\bf4.50\\ \bf4.77} \comment{bursting} \comment{BP} & \makecell{3.00\\3.02} & \makecell{3.60\\3.67} & \makecell{4.32\\4.52} & \makecell{5.19\\5.59} & \makecell{6.25\\6.93} \comment{Our} & \makecell{\bf3.01\\ \bf3.04} & \makecell{\bf3.63\\ \bf3.71} & \makecell{\bf4.37\\ \bf4.58} & \makecell{\bf5.27\\ \bf5.67} & \makecell{\bf6.34\\ \bf7.00} \\ \midrule
% CCSDS(128,64)   \comment{AWGN} \comment{BP} & \makecell{4.32\\4.82} & \makecell{6.46\\7.32} & \makecell{9.61\\10.83} & \makecell{13.99\\ \bf15.43} & \makecell{\bf18.27\\18.51} \comment{Our} & \makecell{\bf4.45\\ \bf5.01} & \makecell{\bf6.66\\ \bf7.59} & \makecell{\bf9.86\\ \bf11.17} & \makecell{\bf14.05\\15.39} & \makecell{18.14\\ \bf18.93} \comment{Fading} \comment{BP} & \makecell{4.37\\4.89} & \makecell{5.72\\6.43} & \makecell{7.42\\8.29} & \makecell{9.47\\10.28} & \makecell{11.84\\12.88} \comment{Our} & \makecell{\bf4.97\\ \bf5.82} & \makecell{\bf6.46\\ \bf7.55} & \makecell{\bf8.23\\ \bf9.52} & \makecell{\bf10.34\\ \bf11.82} & \makecell{\bf12.29\\ \bf13.91} \comment{bursting} \comment{BP} & \makecell{3.62\\3.97} & \makecell{5.29\\5.98} & \makecell{7.81\\8.85} & \makecell{11.25\\12.53} & \makecell{\bf15.59\\ \bf17.10} \comment{Our} & \makecell{\bf4.02\\ \bf4.59} & \makecell{\bf5.86\\ \bf6.84} & \makecell{\bf8.45\\ \bf9.91} & \makecell{\bf11.91\\ \bf13.61} & \makecell{15.34\\17.04} \\ \midrule
% LDPC(121,60)    \comment{AWGN} \comment{BP} & \makecell{3.33\\3.53} & \makecell{4.81\\5.31} & \makecell{7.17\\7.96} & \makecell{10.75\\11.85} & \makecell{15.69\\17.01} \comment{Our} & \makecell{\bf5.18\\ \bf6.07} & \makecell{\bf7.59\\ \bf8.80} & \makecell{\bf10.94\\ \bf12.41} & \makecell{\bf14.65\\ \bf15.25} & \makecell{\bf17.38\\ \bf17.66} \comment{Fading} \comment{BP} & \makecell{3.24\\3.44} & \makecell{4.10\\4.42} & \makecell{5.23\\5.61} & \makecell{6.68\\7.04} & \makecell{8.56\\8.77} \comment{Our} & \makecell{\bf5.32\\ \bf6.23} & \makecell{\bf6.77\\ \bf7.73} & \makecell{\bf8.32\\ \bf9.02} & \makecell{\bf9.61\\ \bf9.96} & \makecell{\bf10.46\\ \bf10.68} \comment{bursting} \comment{BP} & \makecell{2.87\\2.98} & \makecell{3.97\\4.31} & \makecell{5.75\\6.37} & \makecell{8.40\\9.25} & \makecell{12.16\\13.10} \comment{Our} & \makecell{\bf3.66\\ \bf4.08} & \makecell{\bf5.27\\ \bf6.00} & \makecell{\bf7.65\\ \bf8.64} & \makecell{\bf10.95\\ \bf12.10} & \makecell{\bf15.31\\ \bf16.13} \\ \midrule
% LDPC(121,80)    \comment{AWGN} \comment{BP} & \makecell{4.50\\4.50} & \makecell{6.59\\6.60} & \makecell{9.68\\9.66} & \makecell{13.43\\13.91} & \makecell{\bf18.51\\ \bf18.75} \comment{Our} & \makecell{\bf5.15\\ \bf5.15} & \makecell{\bf7.59\\ \bf7.58} & \makecell{\bf10.93\\ \bf11.05} & \makecell{\bf15.34\\ \bf15.19} & \makecell{18.42\\18.53} \comment{Fading} \comment{BP} & \makecell{3.67\\3.89} & \makecell{4.60\\4.97} & \makecell{5.80\\6.29} & \makecell{7.22\\7.82} & \makecell{8.95\\9.58} \comment{Our} & \makecell{\bf4.37\\ \bf4.87} & \makecell{\bf5.53\\ \bf6.23} & \makecell{\bf6.93\\ \bf7.80} & \makecell{\bf8.50\\ \bf9.40} & \makecell{\bf10.10\\ \bf10.90} \comment{bursting} \comment{BP} & \makecell{3.74\\3.94} & \makecell{5.30\\5.81} & \makecell{7.60\\8.50} & \makecell{10.66\\12.15} & \makecell{14.88\\16.45} \comment{Our} & \makecell{\bf4.31\\ \bf4.73} & \makecell{\bf6.23\\ \bf7.00} & \makecell{\bf8.93\\ \bf10.11} & \makecell{\bf12.35\\ \bf13.72} & \makecell{\bf16.02\\ \bf16.98} \\ \midrule
% LDPC(128,64)    \comment{AWGN} \comment{BP} & \makecell{2.88\\3.04} & \makecell{3.66\\4.00} & \makecell{4.65\\5.16} & \makecell{5.80\\6.42} & \makecell{7.03\\7.77} \comment{Our} & \makecell{\bf3.36\\ \bf3.73} & \makecell{\bf4.38\\ \bf4.96} & \makecell{\bf5.55\\ \bf6.35} & \makecell{\bf6.79\\ \bf7.73} & \makecell{\bf7.97\\ \bf9.18} \comment{Fading} \comment{BP} & \makecell{2.73\\2.90} & \makecell{3.22\\3.51} & \makecell{3.80\\4.18} & \makecell{4.44\\4.84} & \makecell{5.14\\5.54} \comment{Our} & \makecell{\bf3.47\\ \bf3.90} & \makecell{\bf4.19\\ \bf4.72} & \makecell{\bf5.00\\ \bf5.60} & \makecell{\bf5.87\\ \bf6.52} & \makecell{\bf6.77\\ \bf7.50} \comment{bursting} \comment{BP} & \makecell{2.58\\2.68} & \makecell{3.23\\3.48} & \makecell{4.08\\4.51} & \makecell{5.09\\5.66} & \makecell{6.21\\6.88} \comment{Our} & \makecell{\bf2.68\\ \bf2.82} & \makecell{\bf3.40\\ \bf3.71} & \makecell{\bf4.31\\ \bf4.78} & \makecell{\bf5.38\\ \bf5.97} & \makecell{\bf6.53\\ \bf7.23} \\ \midrule
% LDPC(32,16)     \comment{AWGN} \comment{BP} & \makecell{3.45\\3.59} & \makecell{4.36\\4.64} & \makecell{5.59\\6.07} & \makecell{7.18\\7.94} & \makecell{9.19\\10.23} \comment{Our} & \makecell{\bf3.60\\ \bf3.78} & \makecell{\bf4.57\\ \bf4.88} & \makecell{\bf5.83\\ \bf6.36} & \makecell{\bf7.49\\ \bf8.22} & \makecell{\bf9.65\\ \bf10.58} \comment{Fading} \comment{BP} & \makecell{3.44\\3.62} & \makecell{4.03\\4.29} & \makecell{4.70\\5.06} & \makecell{5.47\\5.90} & \makecell{6.31\\6.83} \comment{Our} & \makecell{\bf3.87\\ \bf4.11} & \makecell{\bf4.52\\ \bf4.86} & \makecell{\bf5.26\\ \bf5.68} & \makecell{\bf6.07\\ \bf6.55} & \makecell{\bf6.93\\ \bf7.47} \comment{bursting} \comment{BP} & \makecell{3.10\\3.21} & \makecell{3.88\\4.09} & \makecell{4.89\\5.26} & \makecell{6.18\\6.76} & \makecell{7.82\\8.58} \comment{Our} & \makecell{\bf3.23\\ \bf3.37} & \makecell{\bf4.03\\ \bf4.29} & \makecell{\bf5.09\\ \bf5.51} & \makecell{\bf6.43\\ \bf7.07} & \makecell{\bf8.10\\ \bf8.93} \\ \midrule
% LDPC(96,48)     \comment{AWGN} \comment{BP} & \makecell{4.72\\4.72} & \makecell{6.73\\6.71} & \makecell{9.48\\9.47} & \makecell{12.98\\12.77} & \makecell{16.87\\ \bf16.89} \comment{Our} & \makecell{\bf5.02\\ \bf5.02} & \makecell{\bf7.09\\ \bf7.09} & \makecell{\bf9.81\\ \bf9.88} & \makecell{\bf13.32\\ \bf13.43} & \makecell{\bf17.07\\16.85} \comment{Fading} \comment{BP} & \makecell{4.92\\4.91} & \makecell{6.24\\6.25} & \makecell{7.84\\7.82} & \makecell{9.60\\9.57} & \makecell{\bf11.64\\11.44} \comment{Our} & \makecell{\bf4.94\\ \bf4.94} & \makecell{\bf6.27\\ \bf6.26} & \makecell{\bf7.84\\ \bf7.82} & \makecell{\bf9.66\\ \bf9.61} & \makecell{11.48\\ \bf11.53} \comment{bursting} \comment{BP} & \makecell{4.03\\4.40} & \makecell{5.68\\6.33} & \makecell{7.94\\8.91} & \makecell{10.90\\11.99} & \makecell{14.27\\15.55} \comment{Our} & \makecell{\bf4.20\\ \bf4.67} & \makecell{\bf5.88\\ \bf6.68} & \makecell{\bf8.19\\ \bf9.33} & \makecell{\bf11.10\\ \bf12.34} & \makecell{\bf14.33\\ \bf16.17} \\ \midrule
% LTE(132,40)     \comment{AWGN} \comment{BP} & \makecell{2.49\\2.49} & \makecell{2.94\\2.94} & \makecell{3.32\\3.31} & \makecell{3.57\\3.57} & \makecell{3.81\\3.81} \comment{Our} & \makecell{\bf2.66\\ \bf2.66} & \makecell{\bf3.15\\ \bf3.15} & \makecell{\bf3.55\\ \bf3.55} & \makecell{\bf3.86\\ \bf3.86} & \makecell{\bf4.14\\ \bf4.14} \comment{Fading} \comment{BP} & \makecell{2.82\\2.82} & \makecell{3.17\\3.16} & \makecell{3.45\\3.45} & \makecell{3.67\\3.68} & \makecell{3.89\\3.89} \comment{Our} & \makecell{\bf4.11\\ \bf4.10} & \makecell{\bf4.71\\ \bf4.71} & \makecell{\bf5.29\\ \bf5.28} & \makecell{\bf5.84\\ \bf5.83} & \makecell{\bf6.36\\ \bf6.35} \comment{bursting} \comment{BP} & \makecell{2.30\\2.63} & \makecell{2.75\\3.17} & \makecell{3.17\\3.62} & \makecell{3.47\\3.96} & \makecell{3.70\\4.19} \comment{Our} & \makecell{\bf2.35\\ \bf2.70} & \makecell{\bf2.82\\ \bf3.29} & \makecell{\bf3.26\\ \bf3.81} & \makecell{\bf3.59\\ \bf4.18} & \makecell{\bf3.84\\ \bf4.45} \\ \midrule
% MACKAY(96,48)   \comment{AWGN} \comment{BP} & \makecell{4.77\\5.28} & \makecell{6.75\\7.59} & \makecell{9.45\\10.52} & \makecell{12.85\\14.09} & \makecell{16.37\\17.43} \comment{Our} & \makecell{\bf4.89\\ \bf5.48} & \makecell{\bf6.90\\ \bf7.84} & \makecell{\bf9.57\\ \bf10.77} & \makecell{\bf12.90\\ \bf14.37} & \makecell{\bf16.64\\ \bf17.87} \comment{Fading} \comment{BP} & \makecell{4.98\\5.55} & \makecell{6.28\\7.04} & \makecell{\bf7.86\\8.76} & \makecell{\bf9.55\\10.64} & \makecell{11.30\\12.58} \comment{Our} & \makecell{\bf4.98\\ \bf5.55} & \makecell{\bf6.29\\ \bf7.05} & \makecell{7.83\\ \bf8.78} & \makecell{9.53\\ \bf10.66} & \makecell{\bf11.46\\ \bf12.61} \comment{bursting} \comment{BP} & \makecell{4.08\\4.47} & \makecell{5.72\\6.39} & \makecell{7.97\\8.90} & \makecell{10.81\\11.91} & \makecell{13.92\\15.23} \comment{Our} & \makecell{\bf4.26\\ \bf4.75} & \makecell{\bf5.91\\ \bf6.75} & \makecell{\bf8.14\\ \bf9.31} & \makecell{\bf10.94\\ \bf12.35} & \makecell{\bf14.02\\ \bf15.48} \\ \midrule
% POLAR(128,86)   \comment{AWGN} \comment{BP} & \makecell{3.25\\3.36} & \makecell{3.76\\4.02} & \makecell{4.17\\4.67} & \makecell{4.58\\5.38} & \makecell{5.12\\6.19} \comment{Our} & \makecell{\bf3.36\\ \bf3.51} & \makecell{\bf3.96\\ \bf4.28} & \makecell{\bf4.46\\ \bf5.08} & \makecell{\bf4.92\\ \bf5.95} & \makecell{\bf5.54\\ \bf6.91} \comment{Fading} \comment{BP} & \makecell{\bf2.80\\ \bf2.87} & \makecell{\bf3.15\\ \bf3.28} & \makecell{3.53\\3.73} & \makecell{3.91\\4.18} & \makecell{4.26\\4.60} \comment{Our} & \makecell{2.79\\2.86} & \makecell{3.14\\3.28} & \makecell{\bf3.55\\ \bf3.75} & \makecell{\bf3.94\\ \bf4.22} & \makecell{\bf4.30\\ \bf4.66} \comment{bursting} \comment{BP} & \makecell{2.95\\3.02} & \makecell{3.48\\3.65} & \makecell{3.96\\4.31} & \makecell{4.37\\4.97} & \makecell{4.78\\5.66} \comment{Our} & \makecell{\bf3.03\\ \bf3.14} & \makecell{\bf3.65\\ \bf3.89} & \makecell{\bf4.25\\ \bf4.70} & \makecell{\bf4.78\\ \bf5.53} & \makecell{\bf5.30\\ \bf6.35} \\ \midrule
% RS(60,52)       \comment{AWGN} \comment{BP} & \makecell{3.65\\3.70} & \makecell{4.41\\4.54} & \makecell{5.32\\5.52} & \makecell{6.41\\6.64} & \makecell{7.80\\8.04} \comment{Our} & \makecell{\bf3.93\\ \bf3.95} & \makecell{\bf5.00\\ \bf5.06} & \makecell{\bf6.43\\ \bf6.56} & \makecell{\bf8.18\\ \bf8.39} & \makecell{\bf10.22\\ \bf10.52} \comment{Fading} \comment{BP} & \makecell{2.86\\2.87} & \makecell{3.11\\3.13} & \makecell{3.41\\3.43} & \makecell{3.77\\3.81} & \makecell{4.16\\4.24} \comment{Our} & \makecell{\bf2.95\\ \bf2.95} & \makecell{\bf3.26\\ \bf3.27} & \makecell{\bf3.63\\ \bf3.65} & \makecell{\bf4.06\\ \bf4.10} & \makecell{\bf4.52\\ \bf4.59} \comment{bursting} \comment{BP} & \makecell{3.26\\3.27} & \makecell{3.85\\3.91} & \makecell{4.58\\4.72} & \makecell{5.44\\5.67} & \makecell{6.43\\6.78} \comment{Our} & \makecell{\bf3.40\\ \bf3.41} & \makecell{\bf4.15\\ \bf4.19} & \makecell{\bf5.11\\ \bf5.22} & \makecell{\bf6.27\\ \bf6.46} & \makecell{\bf7.50\\ \bf7.77} \\ 
% 		\bottomrule
% 	\end{tabular}
% 	}
% \end{table} 
